MLOD: Awareness of Extrinsic Perturbation in Multi-LiDAR 3D Object Detection for Autonomous Driving

Extrinsic perturbation always exists in multiple sensors. In this paper, we focus on the extrinsic uncertainty in multi-LiDAR systems for 3D object detection. We first analyze the influence of extrinsic perturbation on geometric tasks with two basic examples. To minimize the detrimental effect of extrinsic perturbation, we propagate an uncertainty prior on each point of input point clouds, and use this information to boost an approach for 3D geometric tasks. Then we extend our findings to propose a multi-LiDAR 3D object detector called MLOD. MLOD is a two-stage network where the multi-LiDAR information is fused through various schemes in stage one, and the extrinsic perturbation is handled in stage two. We conduct extensive experiments on a real-world dataset, and demonstrate both the accuracy and robustness improvement of MLOD. The code, data and supplementary materials are available at: https://ram-lab.com/file/site/mlod

==> implementation.tex <==
\section{Implementation Details}
In this section, we explain the implementation details of the MLOD and the training procedure.

\subsection{Network Details}
We set $\alpha=, \beta=, \eta=$ so that $\mathcal{L}_{\text{cls}}^{\text{pos}}$ and $\mathcal{L}_{\text{cls}}^{\text{neg}}$ as well as $\mathcal{L}_{\text{cls}}$ and $\mathcal{L}_{\text{reg}}$ will be of the same orders of magnitude. We first train the network for 100



\subsection{Data Augmentation}

==> methodology_yun.tex <==
\section{Methodology}
\subsection{Problem Definition}
We denote the $i$th LiDAR as $L_i$,
the coordinate frame of $L_i$ as $F_{i}$.
We define a common frame as $F_I$,
and the transformation matrix from $F_i$ to $F_I$ as $T_{Ii} \in \mathbb{R}^{4\times4}$.
We use $P_i$ to represent the point cloud captured from $L_i$,
and $P_i = \{p_i = [x, y, z, 1]^T| i =1, ..., n\}$.
We assume the $T_{Ii}$ subjects to a Gaussian distribution: $T_{Ti} \sim \mathit{N}(\mu, \sigma)$,
and all the LiDARs are well syncronized.

In the multi-LiDAR 3D object detection problem,
the input is a set of point clouds captured by different LiDARs synchronously
$\{P_i^{F_i}, i=1, ..., M\}$, where $M$ are the number of LiDARs.
The goal is to find a set of 3D bounding boxes covering the object of pre-defined classes
as its single-LiDAR counterpart.
A set of 3D bounding boxes is parameterized as $B^{F_I} = \{b_i^{F_I}=[cls, x,y,z,w,l,h,\theta]| i=1,...,m\}$
where $cls$ is the class of the bounding box, 
and $[x,y,z]^{T}$ is the bottom center of the 3D bounding box,
as well as $[w,h,l]$ is the size of the 3D bounding box along the x,y,z-axises respectively 
(x and y axises define the ground plane in the right-handed coordinate system).
$\theta$ is the rotation of the 3D bounding box along the z-axis in range of $(0, \pi]$.

\subsection{Network Architecture}
We employ the network and training scheme described in \cite{Zhou_2018_CVPR,yan2018second}.
The network contains three components: \textbf{FLN} for feature extraction;
\textbf{ML} for feature embedding with sparse convolution;
\textbf{RPN} for box prediction and regression.
We will review the major functions of these components for our further fusion description.

\paragraph{Feature Learning Network}:
The FLN encodes the sparse points into a dense feature representation.
In \cite{Zhou_2018_CVPR}, the authors first voxelize the input point cloud and then applies a bunch of voxel feature encoding layers (VFELayers).
The VFELayer is composed of multi-layer perceptrons and a max-pooling layer.
In the max-pooling layer, the point-wise features inside a voxel are aggregated into voxeli-wise features,
which will be forwarded to ML for feature embedding.
We simplify the FLN in \cite{Zhou_2018_CVPR} by computing the mean value of the points within each voxel as \cite{yan2018second}
\footnote{https://https://github.com/traveller59/second.pytorch}.
A comparable results can be achived if we use the memory saved from simplifying FLN to implement a finer voxelization.

\paragraph{Middle Layers}:
The ML converts the 3D dense grid to a 2D bird's-eye-view (BEV) representation.
To process the grids, the ML is implemented with several 3D convolution layers,
where the 3D convolutional operations,
BN layer, and ReLU layer are applied sequentially.
The convolution kernel size is set as $[d,1,1]$,
since we denote the dense grids in the order of $z,x,y$.
As a result, these layers can aggregate voxel-wise features within a progressively expanding receptive field along the $z\textendash$ axis as well as enrich the shape description. 

In \cite{Zhou_2018_CVPR}, the ML costs almost $50\%$ computation of the whole network due to the dense 3D convolutional operations.
The non-empty voxels usually occupy $\leq 1\%$ of all grids.
However, in the process of dense convolution, calculation is required on each voxel.
Inspired by \cite{yan2018second}, we utilize the spatially sparse convolution \cite{graham2017submanifold} to replace the dense convolution layers in the basic ML.
Hence, the inference time is boosted from $250$ ms approximately to $56$ ms even with larger sampling resolution.

\paragraph{Region Proposal Network}:
The RPN applies convolutional layers to predict the probability and regression map from the extracted features.
Each entry of the probability map estimates the probability of the objectiveness,
and one in the regression map regresses the pose and size of a bounding box.
We jointly estimate $(\sin\theta, \cos\theta)$ instead of $\theta$ to avoid the angular singularity problem described in \cite{simon2018complex}.

\subsection{Fusion of Point Clouds}
According to the stages where the information from multiple LiDARs is fused, we generally propose three fusion schemes, which we call \textit{input fusion}, \textit{feature fusion}, and \textit{result fusion}. These fusion approaches are developed from the above network architecture with several modifications. Fig. \ref{fig.fusion} shows the pipelines of these methods.


\subsubsection{Input Fusion}
\label{sec.input_fusion}
We perform the fusion of point cloud at the input stage.
We project the raw point clouds perceived by all LiDARs into a unified coordinate system
\begin{equation}
\mathcal{P}_{\text{fused}} 
=
(\mathbf{T}_{l^{1}}^{b}\cdot\mathcal{P}_{l^{1}})\oplus
(\mathbf{T}_{l^{2}}^{b}\cdot\mathcal{P}_{l^{2}})\oplus    
\dots \oplus
(\mathbf{T}_{l^{I}}^{b}\cdot\mathcal{P}_{l^{I}}),
\end{equation}
where $I$ is the number of LiDARs used for object detection; the coordinate system $\{l^{i}\}$ and $\{b\}$ are defined as the sensor frame of $i^{th}$ LiDAR and the base frame of the vehicle respectively; the transformation from $\{b\}$ to $\{l^{i}\}$ is denoted by $\mathbf{T}_{l^{1}}^{b}$; the fused point cloud is indicated by $\mathcal{P}_{\text{fused}}$.
$\oplus$ is used to represent a join operation (e.g., projection, summation). As a result,
$\mathcal{P}_{\text{fused}}$ is fed as input into the network.

\subsubsection{Feature Fusion}
\label{sec.feature_fusion}
To enhance the feature interaction, the data are also fused at the feature level. We use the FLN and ML to extract features of each point cloud, and adopt the maximum value to construct a new one as follows
\begin{equation}
\begin{split}
\mathcal{F}_{\text{fused}} 
=
(\mathbf{T}_{l^{1}}^{b}\cdot\mathcal{F}_{l^{1}})\oplus
(\mathbf{T}_{l^{2}}^{b}\cdot\mathcal{F}_{l^{2}})\oplus    
\dots \oplus
(\mathbf{T}_{l^{I}}^{b}\cdot\mathcal{F}_{l^{I}}),         
\end{split}
\end{equation}
where $\mathcal{F}_{l^{i}}$ denotes the resulting features computed by the FLN and ML of $i^{th}$ point cloud. 

\subsubsection{Result Fusion}
\label{sec.result_fusion}
The result fusion scheme takes the resulting bounding boxes and their related points as inputs
and produces a set of refined bounding boxes.
$\mathcal{B}_{l^{i}}$ denotes the set of bounding boxes estimated with the $i^{th}$ LiDAR,
and $\mathcal{B}^{fused}$ denotes the set of refined boxes.
\begin{equation}
\begin{split}
\mathcal{B}_{\text{fused}} 
=
(\mathbf{T}_{l^{1}}^{b}\cdot\mathcal{B}_{l^{1}})\oplus
(\mathbf{T}_{l^{2}}^{b}\cdot\mathcal{B}_{l^{2}})\oplus    
\dots \oplus
(\mathbf{T}_{l^{I}}^{b}\cdot\mathcal{B}_{l^{I}}).     
\end{split}
\end{equation}

After projection, each object may be associated with several candidate boxes.
To reduce redundancy, a basic $\oplus$ operation is non-maximum surppression (NMS) with 3D intersection-over-Union (IoU),
which have been widely applied as a post-processing method\cite{Zhou_2018_CVPR,yan2018second}.d


==> peng.tex <==
\section{Peng's manuscript}


\subsection{Problem Definition}
We denote the $i$th LiDAR as $L_i$,
the coordinate frame of $L_i$ as $F_{i}$.
We define a common frame as $F_I$,
and the transformation matrix from $F_i$ to $F_I$ as $T_{Ii} \in \mathbb{R}^{4\times4}$.
We use $P_i$ to represent the point cloud captured from $L_i$,
and $P_i = \{p_i = [x, y, z, 1]^T| i =1, ..., n\}$.
We assume the $T_{Ii}$ subjects to a Gaussian distribution: $T_{Ti} \sim \mathit{N}(\mu, \sigma)$,
and all the LiDARs are well syncronized.

In the multi-LiDAR 3D object detection problem,
the input is a set of point clouds captured by different LiDARs synchronously
$\{P_i^{F_i}, i=1, ..., M\}$, where $M$ are the number of LiDARs.
The goal is to find a set of 3D bounding boxes covering the object of pre-defined classes
as its single-LiDAR counterpart.
A set of 3D bounding boxes is parameterized as $B^{F_I} = \{b_i^{F_I}=[cls, x,y,z,w,l,h,\theta]| i=1,...,m\}$
where $cls$ is the class of the bounding box, 
and $[x,y,z]^{T}$ is the bottom center of the 3D bounding box,
as well as $[w,h,l]$ is the size of the 3D bounding box along the x,y,z-axises respectively 
(x and y axises define the ground plane in the right-handed coordinate system).
$\theta$ is the rotation of the 3D bounding box along the z-axis in range of $(0, \pi]$.



introduction:
problem: tackling calibration uncertainty in multi-lidar system for 3d object detection
why hard: a gap bridging single-lidar detection to multi-lidar detection, several problems like motion distortion (rolling-shutter scanning), calibration uncertainty (confidence), 

problem analysis
analyze the effect of the calibration uncertainty to detect an object? (be more mathematical)
1. uncertainty propagation
2. point cloud similarity?  an object at increasing distance to the origin?
3. two lidar to observe a clinda, if no uncertainty, two lidar can provides good observation, and fit better curves; but with more calibration uncertainty, the fitting curves may be worse.

methodology
1. first stage
2. second stage
	- network architecture
	- how to incorporate uncertainty value into the network

experiment
1. accuracy against input fusion, feature fusion, result fusion without calibration uncertainty
2. accuracy, robustness under different calibration uncertainty
	- when uncertainty is large, the problem falls into the single lidar detection, should be better or equal to the base line
	- 
	













==> ral_response.tex <==
\section{Response to Reviewers}

\subsection{Why Use Gaussian Noise}

The Gaussian noise model has been widely applied in many linear systems such as the Kailman filter \cite{zarchan2013fundamentals,mourikis2007multi} and SLAM systems using a batch-optimization  formulation \cite{furgale2012continuous,cadena2016past}. 
We consider the input perturbation on the multi-LiDAR systems mainly steaming from sensor noise, vibration, calibration error \cite{brossard2020new}. These factors are either unavoidable or unpredictable in practice, and they are generally linear.
We do not consider the case that the mechanical configuration is manually changed. This process is deterministic and cannot be modeled as a random variable.
Thus, using the Gaussian model is reasonable to describe perturbation in real tests is reasonable. Let us give more details as follows. 

\subsubsection{Sensor Noise} 
As described in \cite{brossard2020new}, the sensor noise consists of the white noise and bias noise. The former affects the precision of each point captured by a LiDAR on a centimeter magnitude. 
The latter stems from temperature drift effect, observed material, incidence and beam angles resulting in large bias, etc. 
They are assumed to be linear and there are extensive works modeling LiDAR measurements as a zero-mean Gaussian distribution \cite{pomerleau2012noise,kruapech2010laser,wang2018characterization,tang2018learning,laconte2019lidar}.

\subsubsection{Vibration}
Vibration on the multi-sensor transformations also exists due to motion \cite{ling2016high,scott2015exploiting}. 
As plotted in Fig. \ref{fig.rep_lyft5_extrinsics}, the provided extrinsics from the LYFT5 dataset are changing over days.
To figure out the distribution of the vibration, there are several works exhaustively conducting the random mechanical vibration tests in laboratories.
And they resulted in the Gaussian model \cite{wang2017comparative}. 
Therefore, we follow the convention to assume the vibration to on the multi-LiDAR systems as Gaussian.
	
\subsubsection{Calibration Uncertainty} 
The calibration uncertainty also contributes to the input perturbation. In many calibration approaches, recovering the multi-LiDAR transformations usually falls into the iterative closest point (ICP) problem. 
As presented in \cite{censi2007accurate,buch2017prediction,landry2019cello,bonnabel2016covariance}, the results of ICP are commonly assumed to be Gaussian. 
Furthermore, we also perform an online calibration on the LYFT5 dataset. Fig. \ref{fig.rep_calibrated_extrinsics} shows the calibrated extrinsics with $1000$ trials. 



\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figure/ral_rebuttle/extrinsics_lyft5_overtime-crop.pdf}
	\caption{Changing extrinsics on the LYFT5 dataset.}
	\label{fig.rep_lyft5_extrinsics}
\end{figure}








==> supplementary_material.tex <==
\section{Supplementary Material}

\subsection{Dataset Details}
We provide the detailed parameters of CARLA for data collection in Tab. \ref{tab.carla_setup}. The whole dataset cover four episodes with different starting points. In each episode, $2000$ frames are collected, and we remove the start frames, so $7944$ frames in total are used for training and evaluation. 

\begin{figure*}
	\centering
	\includegraphics[width=0.66\textwidth]{figure/experiment/carla_car-crop.pdf}
	\caption{The multi-LiDAR setup on the vehicle in CARLA.}  
	\label{fig.carla_car}    
\end{figure*}  

\begin{table*}[tph]
	\centering  	
	\begin{tabular}{ccccc}
		\hline
		\toprule[0.03cm] 
		Episode & Total Frame & $N_{\text{vehicle}}$ & $N_{\text{pedestrain}}$ 
		&\begin{tabular}[c]{@{}c@{}}LiDAR property\\ (range[m], points/s, hz, vertical FOV)\end{tabular}
		\\ \hline \toprule[0.03cm]
		4       & 7944            & 90               & 60                  & $100,\ 250000,\ 10,\ +2 \text{ to } 24.8^{\circ}$ \\ 
		\hline
		\toprule[0.03cm] 
	\end{tabular}
	\caption{The CARLA setup.}	
	\label{tab.carla_setup}       
\end{table*}

We follow \cite{rs_p3} to design the multi-LiDAR setup, which consists of three 64-beam LiDARs mounted on a vehicle. As presented in Fig. \ref{fig.carla_car}, all LiDARs are mounted on the top, and both $l^{2}$ and $l^{3}$ have $30$-degree rotational offsets on the $x\textendash$ axis compared to $l^{1}$. 
Here we use $b\ominus l^{i}$ to represent the configuration from $b$ to $l^{i}$. The extrinsic parameters of different frames are shown in Tab. \ref{tab.real_sensor_setup}.
\begin{table}[tph]
	\centering 
	\renewcommand\arraystretch{0.9}
	\renewcommand\tabcolsep{5pt}    
	\begin{tabular}{ccccccc}
		\hline
		\toprule[0.03cm] 
		{\multirow{2}{*}{Conf.}} & \multicolumn{3}{c}{Rotation {[}degree{]}}                                               & \multicolumn{3}{c}{Translation {[}m{]}}    \\ \cline{2-7} 
		{}                       & x                         & y                         & z                          & x                          & y                         & z                          \\ \hline \toprule[0.03cm]
		$b\ominus l^{1}$  & 0 & 0 & 0 & 0 & 0 & 2.4 \\ 
		$b\ominus l^{2}$  & -30 & 0 & 0 & 0 & 0.8 & 2.2 \\ 
		$b\ominus l^{3}$  & 30 & 0 & 0 &0 & -0.8 & 2.2  \\                 
		\hline
		\toprule[0.03cm] 
	\end{tabular}    
	\label{tab.real_sensor_setup}   
	\caption{The extrinsic parameters of the multi-LiDAR system.}  	  
\end{table}

\newpage
\subsection{Network Details}
The network details for 3D object detection are shown in Tab. \ref{tab.network_details}. The feature learning network (FLN) consists of a fully connected layer, a batch normalization layer and a ReLU layer sequentially.
Each Subm-Conv3D / Sparse-Conv3D block in the Middle Layers (ML) includes a 3D sub-manifold convolution layer/ 3D Sparse convolution layer, a batch normalization layer and a ReLU layer sequentially. 
The Conv2D block in the region proposal network (RPN) consists of a 2D convolution layer, a ReLU layer and a batch normalization layer.
The model of the Probability Map and Regression Map is an individual 2D convolution layer. We adopt the original parameterization method and residual vector for regression from \cite{zhou2018voxelnet}. 
\begin{table}[tph]
	\begin{center}
		\renewcommand\arraystretch{0.9}
		\renewcommand\tabcolsep{3pt}
		\begin{tabular}{ccccc}
			\hline \toprule[0.03cm] 
			Block Name                   & Layer Name            & \begin{tabular}[c]{@{}c@{}}Kernel Size/ \\ Output Unit\end{tabular} & Strides     & Filter \\ \hline \toprule[0.03cm]
			\multirow{3}{*}{FLN}  & VFE                   & 32                                                                 & N/A         & N/A    \\
			& VFE                   & 128                                                                & N/A         & N/A    \\
			& FCN                    & 128                                                                & N/A         & N/A    \\ \hline \toprule[0.01cm]
			\multirow{8}{*}{ML} & Subm-Conv3D $\times$2 & {[}3,3,3{]}                                                        & {[}1,1,1{]} & 16     \\
			& Sparse-Conv3D         & {[}3,3,3{]}                                                        & {[}2,2,2{]} & 32     \\
			& Subm-Conv3D $\times$2 & {[}3,3,3{]}                                                        & {[}1,1,1{]} & 32     \\
			& Sparse-Conv3D         & {[}3,3,3{]}                                                        & {[}2,2,2{]} & 64     \\
			& Subm-Conv3D $\times$3 & {[}3,3,3{]}                                                        & {[}1,1,1{]} & 64     \\
			& Sparse-Conv3D         & {[}3,3,3{]}                                                        & {[}2,2,2{]} & 64     \\
			& Subm-Conv3D $\times$3 & {[}3,3,3{]}                                                        & {[}1,1,1{]} & 64     \\
			& Sparse-Conv3D         & {[}3,1,1{]}                                                        & {[}2,1,1{]} & 64     \\ \hline \toprule[0.01cm] 
			\multirow{9}{*}{RPN}         & Conv2D                & {[}3,3{]}                                                          & {[}2,2{]}   & 128    \\
			& Conv2D$\times$3       & {[}3,3{]}                                                          & {[}1,1{]}   & 128    \\
			& DeConv                & {[}3,3{]}                                                          & {[}1,1{]}   & 256    \\
			& Conv2D                & {[}3,3{]}                                                          & {[}2,2{]}   & 128    \\
			& Conv2D$\times$5       & {[}3,3{]}                                                          & {[}1,1{]}   & 128    \\
			& DeConv                & {[}2,2{]}                                                          & {[}2,2{]}   & 256    \\
			& Conv2D                & {[}3,3{]}                                                          & {[}2,2{]}   & 256    \\
			& Conv2D$\times$5       & {[}3,3{]}                                                          & {[}1,1{]}   & 256    \\
			& DeConv                & {[}4,4{]}                                                          & {[}4,4{]}   & 256    \\ \hline \toprule[0.01cm]
			Prob-Map                     & Conv2D                & {[}1,1{]}                                                          & {[}1,1{]}   & 2      \\
			Reg-Map                      & Conv2D                & {[}1,1{]}                                                          & {[}1,1{]}   & 16     \\ \hline \toprule[0.03cm]
		\end{tabular}
	\end{center}
	\label{tab.network_details}
	\caption{Our Implementation Details.}	
\end{table}

\subsection{Qualitative Results}
We also show more qualitatively results from the baseline and three fusion approaches on the validation set of CARLA object detection in Fig. \ref{fig.qualitative_result_supply}.

\begin{figure*}
	\centering
	\includegraphics[width=1\textwidth]{figure/experiment/result_whole-crop.pdf}
	\caption{Another example detection results of MLOD with all fusion schemes on CARLA validation set. From left to right, top to bottom indicates the detection on: $l^{1}$, $l^{2}$, $l^{3}$, input fusion, feature fusion, and result fusion. The detection is in yellow color, while the ground-truth is in purple color. }  
	\label{fig.qualitative_result_supply}  
\end{figure*} 




